A new $H_0$ measurement with SNe Requiem and Encore using $\texttt{Gravity.jl}$

We present a strong-lensing (SL) analysis of the galaxy cluster MACS J0138.0-2155 (z=0.336), the first known lens cluster discovered to host two distinct multiply imaged Type Ia supernovae (SNe): SN Requiem and SN Encore. Both SNe are located in the massive, multiply imaged red galaxy MRG-M0138 at z=1.949. The projected total mass of this cluster has been investigated with several independent lens models (Suyu+26; Pierel+26), using a sample of 23 spectroscopically confirmed multiple images from 8 background sources (0.767<z<3.420), identified from HST and JWST imaging data, and VLT/MUSE spectroscopy. In this work, we develop a new SL model based on a novel Bayesian parametric lens-modelling framework $\texttt{Gravity jl}$, exploiting the same SL dataset. Our reference mass model accurately reproduces the observed image positions, with an image-plane rms image position residual of 0.15''. Assuming H0 = 70 km/s/Mpc, we predict the future reappearances of highly delayed SNe counter-images, finding $D_t(1d,1a) = 3122_{-70}^{+75}$ d (April-August 2032) for SN Encore and $D_t(2d,2a) = 3902_{-67}^{+72}$ d (January-May 2027) for SN Requiem. By allowing H0 to vary, and using the measured time delays of SN Encore and Requiem together with their statistical uncertainties as observables, we infer the value of H0 jointly with the other lens-model free parameters, by combining the values inferred from 3 mass models. We obtain a new measurement of $H_0 = 69.2_{-8.0}^{+9.6}$ km/s/Mpc, consistent with the value inferred from independent lens models. This error is currently dominated by the large relative uncertainty on the measured time delays (>10%). The forthcoming reappearance of SN Requiem offers an immediate opportunity to significantly improve constraints on H0, provided that lens-model systematics are controlled. These results establish M0138 as a premier anchor for high-precision cluster TDC.

==> Makefile <==
# Document versions
VERSION := 4
BNAME   := main-v
OLD     := $(shell expr $(VERSION) - 1)

# Current file and old version
FNAME   := $(BNAME)$(VERSION)
OLDDIR  := old
ONAME   := $(OLDDIR)/$(BNAME)$(OLD)

TARGET      := $(FNAME).pdf
DIFF_SOURCE := diff.tex
DIFF_TARGET := diff.pdf

# Programs
LATEXMK  := latexmk
DIFFTEX  := latexdiff

# Preserve standard TeX search paths while adding local directories
export TEXINPUTS := .:sty:

LATEXMK_FLAGS := -pdf -interaction=nonstopmode -file-line-error

DIFF_FLAGS := \
		--graphics-markup=none \
		--disable-citation-markup \
		--exclude-textcmd=texttt \
		--flatten \
		--append-textcmd=abstract

# Rebuild when these inputs change
TEX_SOURCES := $(wildcard *.tex)
BIB_SOURCES := $(wildcard *.bib)
STY_SOURCES := $(wildcard sty/*.sty)
FIGURES     := $(wildcard fig/*)

.PHONY: all diff clean veryclean view xview

all: $(TARGET)

$(TARGET): $(TEX_SOURCES) $(BIB_SOURCES) $(STY_SOURCES) $(FIGURES)
	$(LATEXMK) $(LATEXMK_FLAGS) $(FNAME).tex

# Write to a temporary file first so a failed latexdiff run does not
# leave behind an empty or truncated diff.tex.
$(DIFF_SOURCE): $(ONAME).tex $(FNAME).tex
	$(DIFFTEX) $(DIFF_FLAGS) $(ONAME).tex $(FNAME).tex > $@.tmp
	mv $@.tmp $@

$(DIFF_TARGET): $(DIFF_SOURCE) $(BIB_SOURCES) $(STY_SOURCES) $(FIGURES)
	$(LATEXMK) $(LATEXMK_FLAGS) -f $(DIFF_SOURCE) || test -f $@

diff: $(DIFF_TARGET)

clean:
	-$(LATEXMK) -c $(FNAME).tex
	-$(LATEXMK) -c $(DIFF_SOURCE)
	$(RM) $(DIFF_SOURCE).tmp
	$(RM) *.spl *.tdo *.vrb *Notes.bib

veryclean: clean
	$(RM) $(TARGET) $(DIFF_TARGET) $(DIFF_SOURCE)

view: $(TARGET)
	open -a "Skim.app" "$(TARGET)"

xview: $(TARGET)
	evince "$(TARGET)" >/dev/null 2>&1 &
